s-LIME: Reconciling Locality and Fidelity in Linear Explanations

The benefit of locality is one of the major premises of LIME, one of the most prominent methods to explain black-box machine learning models. This emphasis relies on the postulate that the more locally we look at the vicinity of an instance, the simpler the black-box model becomes, and the more accurately we can mimic it with a linear surrogate. As logical as this seems, our findings suggest that, with the current design of LIME, the surrogate model may degenerate when the explanation is too local, namely, when the bandwidth parameter $\sigma$ tends to zero. Based on this observation, the contribution of this paper is twofold. Firstly, we study the impact of both the bandwidth and the training vicinity on the fidelity and semantics of LIME explanations. Secondly, and based on our findings, we propose \slime, an extension of LIME that reconciles fidelity and locality.

==> related-work.tex <==
%In Section~\ref{subsec:linear-explanations} we first introduce the general principle of explanations based on linear attribution. This sets the ground to survey the most relevant works in this domain.
\subsection{LIME}
\label{subsec:lime}
In \cite{lime}, the authors introduce LIME, a model-agnostic method to explain ML models via linear surrogates. LIME learns an explanation $g$ for a black box $f$ in the vicinity of a point $x$ (with $\eta(x) = \hat{x}$) by solving the following minimization problem:
\[ g = \mathit{argmin}_{g \in \mathcal{G}}{\;\mathcal{L}(f, g, \pi_{\hat{\mathcal{X}}})} + \Omega(g) \]
\noindent That is, the linear surrogate $g$ is chosen such that it minimizes the error $\mathcal{L}$ with respect to the answers of the black box $f$ on a weighted neighborhood $\hat{\mathcal{X}}$ around a target instance $x$. The neighbors $\hat{\mathcal{X}} \subset \{0, 1\}^{\hat{d}}$ lie on a binary space defined on the presence or absence of surrogate features. For instance, if the black-box $f$ represents text instances $x \in \mathbb{R}^d$ using word embeddings, $\eta$ maps $x$ to a binary vector $\hat{x} \in \{0, 1\}^{d'}$ on the absence and presence of individual words.  The weights of the neighbors in $\hat{\mathcal{X}}$ are determined by the kernel function $\pi_{\hat{\mathcal{X}}}$. The expression $\Omega(g)$ is a regularization term that penalizes complex surrogate models. 

LIME sets $\mathcal{L}$ to a locally weighted squared loss, the neighborhood $\hat{\mathcal{X}}$ to (a sample of) the subspace of vectors consisting of subsets of $\hat{x}$'s non-zero components, $\pi_{\hat{x}}$ to an exponentially decreasing kernel on a distance metric $D$, and $\Omega$ to a function that penalizes linear models with more than $k$ non-zero coefficients, that is:

\begin{minipage}{0.6\linewidth}  
%\begin{small}  
\[ \mathcal{L}(f, g, \pi_{\hat{\mathcal{X}}}) = \sum_{\hat{z} \in \mathcal{X}}{\pi_{\hat{\mathcal{X}}}(\hat{z})(f(\eta^{-1}(\hat{z})) - g(\hat{z}))^2} \] 
%\end{small}
\end{minipage}
\begin{minipage}{0.4\linewidth}
%	\begin{small}
\[ \hat{\mathcal{X}} \subseteq \{ \hat{z} \in \{0, 1\}^{\hat{d}} : \mathbbm{1}[\neg \hat{z} \lor \hat{x}] \} \]
%	\end{small}
\end{minipage}
\begin{minipage}{0.5\linewidth}
%\begin{small}
\[ \Omega(g) = \infty \mathbbm{1}\lbrack\;||\bm{\hat{\alpha}} ||_0 > k \; \rbrack \]	
%\end{small}
\end{minipage}
\begin{minipage}{0.5\linewidth}
%\begin{small}
\[ \;\;\;\;\;\;\;\;\;\;\;\;\;\;\pi_{\hat{x}}(\hat{z}) = \mathit{exp}(\nicefrac{-D(\hat{x}, \hat{z})^2}{\sigma^2})\]
%\end{small}
\end{minipage}
\\

\noindent The neighbors in $\hat{\mathcal{X}}$ are obtained by toggling off bits in the target's binary representation $\hat{x}$. According to~\cite{lime}, a bit set to zero in the surrogate space could be mapped back to the original space by removing the corresponding word for text instances, or by replacing a super-pixel by a baseline grayed out segment for images\footnote{Some other alternatives are proposed in \cite{anchors}}.

LIME does not make any assumptions about $f$, however the conversion function $\eta$ depends on $f$'s original space, which at the same time depends on the instances' data type (images, text, or tabular data). 
 Moreover,~\cite{lime} does not discuss about the influence of other arguments such that the bandwidth $\sigma$, the distance $D$, or the neighborhood \neighbors. 

A recent study~\cite{explaining-lime} on LIME explanations proves that if the black box is a linear function, i.e., $f(x) = \alpha_0 + \sum_{1 \le i \le d}{\alpha_i x_i}$, the coefficients $\hat{\alpha}_i$ learned by the tabular non-regularized version of LIME\footnote{That is, when $\Omega(g) = 0$} are proportional to $f$'s gradient $\nabla{}f$, that is the coefficients $\alpha_i$. The proportionality constants are sensitive to the target instance, $\sigma$, the mean and variance of $\hat{\mathcal{X}}$, and the discretization intervals of the original features according to $\eta$. Furthermore,~\cite{explaining-lime} shows the stability of tabular LIME for large sample sizes $n = |\hat{\mathcal{X}}|$, and provides an upper bound for the error of $g$. Despite these positive results,~\cite{explaining-lime} shows empirically that arbitrary choices of $\sigma$ can lead to degenerated explanations where some features are erroneously assigned a null contribution. In this paper we study in detail under which circumstances this phenomenon arises, and propose solutions to avoid it.

%\subsection{DeepLIFT}
%\label{subsec:deeplift}
%DeepLIFT~\cite{deeplift} is an approach to explain the individual influence of the input features in the output of a neural network. In contrast to LIME, DeepLift estimates the contribution of the features to the discrete gradient $\Delta f$ of the black box $f$ on a target $x$. In other words, the weights learned by DeepLIFT respect the \emph{summation-to-delta} invariance:
%\[ \sum_{1 \le i \le \hat{d}}{\hat{\alpha_i}\hat{x}[i]} = \Delta f(x) = f(x) - f(x_{\emptyset}) \]  

%\noindent This gradient is defined with respect to a reference instance $x_{\emptyset}$ and is learned by back-propagating the contribution of all neurons in the network to the input neurons.
%The reference $x_{\emptyset}$ denotes the \emph{no-signal} or \emph{default} scenario, and is context-dependent. Applications for image classification, e.g., could set $x_{\emptyset}$ to a fully black image or to an image with pure salt-and-pepper noise. ML model on texts could likewise set the reference to the zero embedding (empty text). In this spirit, the conversion function $\eta: \mathbb{R}^d \rightarrow \{0, 1\}^{\hat{d}}$ with $d = \hat{d}$, assigns a value of zero to the $i$-th interpretable feature if $x[i]$ takes the value of the reference, i.e., if $x[i] = x_{\emptyset}[i]$. This also entails that $\eta(x_{\emptyset})= \hat{x}_{\emptyset} = \bm{0}^{\hat{d}}$. 

%\subsection{Integrated Gradients}
%In~\cite{ig}, the authors argue that discrete gradients do not satisfy some desirable properties such as the \emph{implementation invariance}. In other words, discrete gradients can differ significantly for two functionally equivalent neural networks with different internal architectures. On those grounds, \cite{ig} proposes Integrated Gradients (IG), a method to estimate the \emph{continuous} gradient $\nabla{}f(x)$ of a black box $f$ on a target $x$ w.r.t. to a reference $x_{\emptyset}$. The weights learned by IG respect the implementation and the summation-to-delta invariances. For this purpose, IG calculates the path integral between $x$ and $x_{\emptyset}$. If $\bm{\alpha}_g$ denotes the vector of coefficients of the surrogate $g$ and $\Delta x = x - x_{\emptyset}$, it follows that,   
%\[\bm{\alpha}_g = \Delta x \times  \int_{0}^{1}{\frac{\partial f(x_{\emptyset} + \gamma \Delta x)}{\partial \gamma} }  \partial \gamma 
%\]

%\subsection{SHAP}

%Gradient-based methods assume the black-box model is differentiable almost everywhere\footnote{Except on a set of isolated points, i.e., subspaces with zero Lesbergue measure.}. Hence, the meaning of the feature contributions computed by those methods is not well-defined for piece-wise constant functions such as trees or forests. A fully model-agnostic way to estimate such contributions w.r.t., a reference instance is given by the Shapley values as proposed by SHAP~\cite{shap}. The Shapley value $\hat{\alpha}_i$ of the $i$-th feature of an instance $x$ is defined as the average difference $\Delta f$ among all possible feature coalitions $S \in 2^{\{1, \dots, n \}}$ when $i$ is present and absent, namely,

%\begin{minipage}{0.55\linewidth}  
%\[ \hat{\alpha}_i = \sum_{S \subset F \setminus \{ i \}}{\beta_S \times f_{S \cup \{ i\} }(x_{S \cup \{ i\}}) - f_S(x_S)}
%\]
%\end{minipage}
%\begin{minipage}{0.45\linewidth}
%\[ \beta_S = \frac{|S|!(|F| - |S| - 1)!}{|F|!} \]	
%\end{minipage}
%\\

%\noindent The notations $f_{S}$ and $x_{S}$ denote partial functions and instances where only the features in $S$ are present. The Shapley values induce a surrogate local model of the form $g(\hat{x}) = f_{\emptyset}(x_{\emptyset}) + \sum_{1 \le i \le n}{\hat{\alpha_i}\hat{x}[i]}$, which means they satisfy the summation-to-delta invariance w.r.t. a reference instance $x_{\emptyset}$ where $\Delta f(x) = f(x) - f_{\emptyset}(x_\emptyset)$. The term $f_{\emptyset}(x_\emptyset)$ is the result of evaluating the reference instance on a model $f_{\emptyset}$ with zero-information. Albeit model-agnostic, SHAP's general formulation is intractable and requires the definition of partial functions and a reference instance. That said, the Shapley values can be efficiently approximated.~\cite{shap} describes several variants of SHAP optimized for particular black-box models such as trees and neural networks.

%\subsection{Non-linear Explanations}
%Explanations for black-box models can also take the form of rules~\cite{anchors} or decision trees \cite{lore}. Anchors~\cite{anchors} is a model-agnostic approach that computes local rule explanations -- named anchors --  for classifiers. These explanations take the form: 
%\[ \bigwedge_{j \in F \subseteq \{1, \dots, \hat{d} \}}{\hat{z}[j]} \Rightarrow f(z) = f(x) \] 
%\noindent This rule describes a set of conditions (on the surrogate space) that \emph{anchor} the black box to the class predicted for the target instance $x$ with high probability. Since multiple anchors may predict $f(x)$ accurately, ~\cite{anchors} reports those with the highest coverage, otherwise speaking, the least local. Hence, anchors are conceptually discrete surrogates of the form $g(\hat{x}) = f(x) + \beta \times (1 - \prod_{j \in F}{\hat{x}[j]})$ that convey the minimal set of variable interactions that guarantee the prediction of $f(x)$ in the largest locality. In contrast to linear explanations, anchors provide a crisp definition of locality.

%LORE \cite{lore} proposes regression trees as local surrogates to explain black-box classifiers on tabular data. The decision trees are induced from a neighborhood sampled using a genetic algorithm on the original space. With this sampling strategy, a neighbor $z$ can be obtained, e.g., by applying a cross-over operator on the target instance $x$, that is, by replacing the value of $x[i]$ with $z'[i]$, for some random $z'$ in the training set. The resulting decision trees can then be used to provide anchor-like explanations for $f(x)$ enhanced with counter-factual explanations. These describe the minimal set of changes required in the features of an instance in order to change $f$'s answer. Although the neighbors are computed in the original space, the decision tree discretizes the original features, thus it also lies on a surrogate space.

